A Theoretical Understanding of Chain-of-Thought: Coherent Reasoning and Error-Aware Demonstration

Few-shot Chain-of-Thought (CoT) prompting has demonstrated strong performance in improving the reasoning capabilities of large language models (LLMs). While theoretical investigations have been conducted to understand CoT, the underlying transformer used in these studies isolates the CoT reasoning process into separated in-context learning steps (Stepwise ICL). In this work, we theoretically show that, compared to Stepwise ICL, the transformer gains better error correction ability and more accurate predictions if the reasoning from earlier steps (Coherent CoT) is integrated. Given that this coherent reasoning changes the behavior of the transformer, we further investigate the sensitivity of the transformer with Coherent CoT when the demonstration examples are corrupted at the inference stage. Our theoretical results indicate that the transformer is more sensitive to errors in intermediate reasoning steps than the final outcome. Building upon this observation, we propose an improvement on CoT by incorporating both correct and incorrect reasoning paths in the demonstration. Our experiments validate the effectiveness of the proposed approach.

==> reference.tex <==

@article{chen2024training,
  title={Training dynamics of multi-head softmax attention for in-context learning: Emergence, convergence, and optimality},
  author={Chen, Siyu and Sheen, Heejune and Wang, Tianhao and Yang, Zhuoran},
  journal={arXiv preprint arXiv:2402.19442},
  year={2024}
}
@article{xing2024benefits,
  title={Benefits of transformer: In-context learning in linear regression tasks with unstructured data},
  author={Xing, Yue and Lin, Xiaofeng and Suh, Namjoon and Song, Qifan and Cheng, Guang},
  journal={arXiv preprint arXiv:2402.00743},
  year={2024}
}
@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom B},
  journal={arXiv preprint arXiv:2005.14165},
  year={2020}
}
@article{bai2023transformers,
  title={Transformers as Statisticians: Provable In-Context Learning with In-Context Algorithm Selection},
  author={Bai, Yu and Chen, Fan and Wang, Huan and Xiong, Caiming and Mei, Song},
  journal={arXiv preprint arXiv:2306.04637},
  year={2023}
}
@inproceedings{dai2023can,
  title={Why Can GPT Learn In-Context? Language Models Implicitly Perform Gradient Descent as Meta-Optimizers},
  author={Dai, Damai and Sun, Yutao and Dong, Li and Hao, Yaru and Ma, Shuming and Sui, Zhifang and Wei, Furu},
  booktitle={ICLR 2023 Workshop on Mathematical and Empirical Understanding of Foundation Models},
  year={2023}
}
@article{cheng2023transformers,
  title={Transformers Implement Functional Gradient Descent to Learn Non-Linear Functions In Context},
  author={Cheng, Xiang and Chen, Yuxin and Sra, Suvrit},
  journal={arXiv preprint arXiv:2312.06528},
  year={2023}
}
@article{cobbe2021training,
  title={Training verifiers to solve math word problems},
  author={Cobbe, Karl and Kosaraju, Vineet and Bavarian, Mohammad and Chen, Mark and Jun, Heewoo and Kaiser, Lukasz and Plappert, Matthias and Tworek, Jerry and Hilton, Jacob and Nakano, Reiichiro and others},
  journal={arXiv preprint arXiv:2110.14168},
  year={2021}
}
@article{srivastava2022beyond,
  title={Beyond the imitation game: Quantifying and extrapolating the capabilities of language models},
  author={Srivastava, Aarohi and Rastogi, Abhinav and Rao, Abhishek and Shoeb, Abu Awal Md and Abid, Abubakar and Fisch, Adam and Brown, Adam R and Santoro, Adam and Gupta, Aditya and Garriga-Alonso, Adri{\`a} and others},
  journal={arXiv preprint arXiv:2206.04615},
  year={2022}
}
@article{bi2024deepseek,
  title={Deepseek llm: Scaling open-source language models with longtermism},
  author={Bi, Xiao and Chen, Deli and Chen, Guanting and Chen, Shanhuang and Dai, Damai and Deng, Chengqi and Ding, Honghui and Dong, Kai and Du, Qiushi and Fu, Zhe and others},
  journal={arXiv preprint arXiv:2401.02954},
  year={2024}
}
@article{team2023gemini,
  title={Gemini: a family of highly capable multimodal models},
  author={Team, Gemini and Anil, Rohan and Borgeaud, Sebastian and Wu, Yonghui and Alayrac, Jean-Baptiste and Yu, Jiahui and Soricut, Radu and Schalkwyk, Johan and Dai, Andrew M and Hauth, Anja and others},
  journal={arXiv preprint arXiv:2312.11805},
  year={2023}
}
@article{huang2023context,
  title={In-context convergence of transformers},
  author={Huang, Yu and Cheng, Yuan and Liang, Yingbin},
  journal={arXiv preprint arXiv:2310.05249},
  year={2023}
}
@article{zhang2023trained,
  title={Trained transformers learn linear models in-context},
  author={Zhang, Ruiqi and Frei, Spencer and Bartlett, Peter L},
  journal={arXiv preprint arXiv:2306.09927},
  year={2023}
}
@article{li2024chain,
  title={Chain of thought empowers transformers to solve inherently serial problems},
  author={Li, Zhiyuan and Liu, Hong and Zhou, Denny and Ma, Tengyu},
  journal={arXiv preprint arXiv:2402.12875},
  year={2024}
}
@article{prystawski2024think,
  title={Why think step by step? Reasoning emerges from the locality of experience},
  author={Prystawski, Ben and Li, Michael and Goodman, Noah},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}
@article{wei2022chain,
  title={Chain-of-thought prompting elicits reasoning in large language models},
  author={Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny and others},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={24824--24837},
  year={2022}
}
@article{kojima2022large,
  title={Large language models are zero-shot reasoners},
  author={Kojima, Takeshi and Gu, Shixiang Shane and Reid, Machel and Matsuo, Yutaka and Iwasawa, Yusuke},
  journal={Advances in neural information processing systems},
  volume={35},
  pages={22199--22213},
  year={2022}
}
@article{fu2023chain,
  title={Chain-of-Thought Hub: A Continuous Effort to Measure Large Language Models' Reasoning Performance},
  author={Fu, Yao and Ou, Litu and Chen, Mingyu and Wan, Yuhao and Peng, Hao and Khot, Tushar},
  journal={arXiv preprint arXiv:2305.17306},
  year={2023}
}
@article{feng2023towards,
  title={Towards Revealing the Mystery behind Chain of Thought: a Theoretical Perspective},
  author={Feng, Guhao and Gu, Yuntian and Zhang, Bohang and Ye, Haotian and He, Di and Wang, Liwei},
  journal={arXiv preprint arXiv:2305.15408},
  year={2023}
}
@article{tutunov2023can,
  title={Why Can Large Language Models Generate Correct Chain-of-Thoughts?},
  author={Tutunov, Rasul and Grosnit, Antoine and Ziomek, Juliusz and Wang, Jun and Bou-Ammar, Haitham},
  journal={arXiv preprint arXiv:2310.13571},
  year={2023}
}
@article{jiang2023latent,
  title={A latent space theory for emergent abilities in large language models},
  author={Jiang, Hui},
  journal={arXiv preprint arXiv:2304.09960},
  year={2023}
}
@article{li2023dissecting,
  title={Dissecting Chain-of-Thought: A Study on Compositional In-Context Learning of MLPs},
  author={Li, Yingcong and Sreenivasan, Kartik and Giannou, Angeliki and Papailiopoulos, Dimitris and Oymak, Samet},
  journal={arXiv preprint arXiv:2305.18869},
  year={2023}
}
@article{cui2024superiority,
  title={Superiority of multi-head attention in in-context linear regression},
  author={Cui, Yingqian and Ren, Jie and He, Pengfei and Tang, Jiliang and Xing, Yue},
  journal={arXiv preprint arXiv:2401.17426},
  year={2024}
}
@article{wang2022self,
  title={Self-consistency improves chain of thought reasoning in language models},
  author={Wang, Xuezhi and Wei, Jason and Schuurmans, Dale and Le, Quoc and Chi, Ed and Narang, Sharan and Chowdhery, Aakanksha and Zhou, Denny},
  journal={arXiv preprint arXiv:2203.11171},
  year={2022}
}
@article{zhang2022automatic,
  title={Automatic chain of thought prompting in large language models},
  author={Zhang, Zhuosheng and Zhang, Aston and Li, Mu and Smola, Alex},
  journal={arXiv preprint arXiv:2210.03493},
  year={2022}
}
@article{chu2023survey,
  title={A survey of chain of thought reasoning: Advances, frontiers and future},
  author={Chu, Zheng and Chen, Jingchang and Chen, Qianglong and Yu, Weijiang and He, Tao and Wang, Haotian and Peng, Weihua and Liu, Ming and Qin, Bing and Liu, Ting},
  journal={arXiv preprint arXiv:2309.15402},
  year={2023}
}
@article{besta2024topologies,
  title={Topologies of Reasoning: Demystifying Chains, Trees, and Graphs of Thoughts},
  author={Besta, Maciej and Memedi, Florim and Zhang, Zhenyu and Gerstenberger, Robert and Blach, Nils and Nyczyk, Piotr and Copik, Marcin and Kwa{\'s}niewski, Grzegorz and M{\"u}ller, J{\"u}rgen and Gianinazzi, Lukas and others},
  journal={arXiv preprint arXiv:2401.14295},
  year={2024}
}
@article{yao2023tree,
  title={Tree of thoughts: Deliberate problem solving with large language models},
  author={Yao, Shunyu and Yu, Dian and Zhao, Jeffrey and Shafran, Izhak and Griffiths, Thomas L and Cao, Yuan and Narasimhan, Karthik},
  journal={arXiv preprint arXiv:2305.10601},
  year={2023}
}
@article{besta2023graph,
  title={Graph of thoughts: Solving elaborate problems with large language models},
  author={Besta, Maciej and Blach, Nils and Kubicek, Ales and Gerstenberger, Robert and Gianinazzi, Lukas and Gajda, Joanna and Lehmann, Tomasz and Podstawski, Michal and Niewiadomski, Hubert and Nyczyk, Piotr and others},
  journal={arXiv preprint arXiv:2308.09687},
  year={2023}
}
@article{garg2022can,
  title={What can transformers learn in-context? a case study of simple function classes},
  author={Garg, Shivam and Tsipras, Dimitris and Liang, Percy S and Valiant, Gregory},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={30583--30598},
  year={2022}
}
@inproceedings{von2023transformers,
  title={Transformers learn in-context by gradient descent},
  author={Von Oswald, Johannes and Niklasson, Eyvind and Randazzo, Ettore and Sacramento, Jo{\~a}o and Mordvintsev, Alexander and Zhmoginov, Andrey and Vladymyrov, Max},
  booktitle={International Conference on Machine Learning},
  pages={35151--35174},
  year={2023},
  organization={PMLR}
}
@article{tang2023large,
  title={Large Language Models are In-Context Semantic Reasoners rather than Symbolic Reasoners},
  author={Tang, Xiaojuan and Zheng, Zilong and Li, Jiaqi and Meng, Fanxu and Zhu, Song-Chun and Liang, Yitao and Zhang, Muhan},
  journal={arXiv preprint arXiv:2305.14825},
  year={2023}
}
@article{wu2023analyzing,
  title={Analyzing chain-of-thought prompting in large language models via gradient-based feature attributions},
  author={Wu, Skyler and Shen, Eric Meng and Badrinath, Charumathi and Ma, Jiaqi and Lakkaraju, Himabindu},
  journal={arXiv preprint arXiv:2307.13339},
  year={2023}
}
@article{wang2022towards,
  title={Towards understanding chain-of-thought prompting: An empirical study of what matters},
  author={Wang, Boshi and Min, Sewon and Deng, Xiang and Shen, Jiaming and Wu, You and Zettlemoyer, Luke and Sun, Huan},
  journal={arXiv preprint arXiv:2212.10001},
  year={2022}
}
@article{madaan2022text,
  title={Text and patterns: For effective chain of thought, it takes two to tango},
  author={Madaan, Aman and Yazdanbakhsh, Amir},
  journal={arXiv preprint arXiv:2209.07686},
  year={2022}
}
@article{lyu2023faithful,
  title={Faithful chain-of-thought reasoning},
  author={Lyu, Qing and Havaldar, Shreya and Stein, Adam and Zhang, Li and Rao, Delip and Wong, Eric and Apidianaki, Marianna and Callison-Burch, Chris},
  journal={arXiv preprint arXiv:2301.13379},
  year={2023}
}

@misc{openai_o1_2024,
  title = {OpenAI o1},
  author = {{OpenAI}},
  year = {2024},
  url = {https://openai.com/o1/},
  note = {Accessed: 2024-10-09}
}
@article{jin2024impact,
  title={The Impact of Reasoning Step Length on Large Language Models},
  author={Jin, Mingyu and Yu, Qinkai and Zhao, Haiyan and Hua, Wenyue and Meng, Yanda and Zhang, Yongfeng and Du, Mengnan and others},
  journal={arXiv preprint arXiv:2401.04925},
  year={2024}
}
@misc{openai_learning_to_reason_2024,
  title = {Learning to Reason with LLMs},
  author = {{OpenAI}},
  year = {2024},
  url = {https://openai.com/index/learning-to-reason-with-llms/},
  note = {Accessed: 2024-10-09}
}

@article{akyurek2022learning,
  title={What learning algorithm is in-context learning? investigations with linear models},
  author={Aky{\"u}rek, Ekin and Schuurmans, Dale and Andreas, Jacob and Ma, Tengyu and Zhou, Denny},
  journal={arXiv preprint arXiv:2211.15661},
  year={2022}
}

@article{ahn2023transformers,
  title={Transformers learn to implement preconditioned gradient descent for in-context learning},
  author={Ahn, Kwangjun and Cheng, Xiang and Daneshmand, Hadi and Sra, Suvrit},
  journal={arXiv preprint arXiv:2306.00297},
  year={2023}
}
